Star formation in IRDC G31.97+0.07

We utilize multiple-waveband continuum and molecular-line data of CO isotopes, to study the dynamical structure and physical properties of the IRDC G31.97+0.07. We derive the dust temperature and H$_2$ column density maps of the whole structure by SED fitting. The total mass is about $2.5\times10^5\,M_{\odot}$ for the whole filamentary structure and about $7.8\times10^4\,M_{\odot}$ for the IRDC. Column density PDFs produced from the column density map are generally in the power-law form suggesting that this part is mainly gravity-dominant. The flatter slope of the PDF of the IRDC implies that it might be compressed by an adjacent, larger \HII region. There are 27 clumps identified from the 850\,\micron \ continuum located in this filamentary structure. Based on the average spacing of the fragments in the IRDC, we estimate the age of the IRDC. The age is about $6.4\,$Myr assuming inclination angle $i = 30^\circ$. For 18 clumps with relatively strong CO and $^{13}$CO (3-2) emission, we study their line profiles and stabilities. We find 5 clumps with blue profiles which indicate gas infall motion and 2 clumps with red profiles which indicate outflows or expansion. Only one clump has $\alpha_\mathrm{vir} > 2$, suggesting that most clumps are gravitationally bound and tend to collapse. In the Mass-$R_\mathrm{eq}$ diagram, 23 of 27 clumps are above the threshold for high-mass star formation, suggesting that this region can be a good place for studying high-mass star-forming.

==> Catalogue/PDF_para.tex <==
\begin{table*}
	\caption{Parameters of the one/two lognormal fits of the PDFs in Figure~\ref{fig:PDF} with the corresponding reduced $\chi^2$ values, and the exponents of the power law fits at high column densities.}
    \label{tab:PDF_para}
\begin{tabular}{cccccccccc}
\hline
Region & $\eta_1$ & $p_1$ & $\sigma_1$ & $\eta_2$ & $p_2$ & $\sigma_2$ & $\chi^2$ & m \\
\hline
1 (two lognormal fit) &-0.73&0.84&0.98&-0.46&0.07&0.18&127&-0.83\\
1 (one lognormal fit) &-0.67&0.87&0.85&...&...&...&141&-0.83\\
%2 &-0.47&0.98&0.94&...&...&...&...\\
3 (one lognormal fit)&-0.06&0.91&1.04&...&...&...&37&-0.78\\
\hline
\end{tabular}
\end{table*}


==> Catalogue/evo_stage.tex <==
\begin{table*}
\caption{evo\_stage}
\begin{tabular}{ccccc}
\hline \\
JPS\_name & Glon & Glat & Associated with YSO & emission in 70$\mu$m \\
\hline \\
JPSG031.925+00.083 & 31.921 & 0.084 & ... & N \\
JPSG031.929+00.056 & 31.927 & 0.057 & ... & N \\
JPSG031.933+00.090 & 31.934 & 0.093 & ... & N \\
JPSG031.945+00.076 & 31.943 & 0.078 & ... & N \\
JPSG031.951+00.071 & 31.950 & 0.070 & ... & N \\
JPSG031.961+00.066 & 31.958 & 0.069 & ... & N \\
JPSG031.965+00.062 & 31.964 & 0.062 & ... & N \\
JPSG031.970+00.060 & 31.971 & 0.059 & ... & N \\
JPSG031.984+00.065 & 31.982 & 0.066 & ... & N \\
JPSG031.991+00.067 & 31.991 & 0.068 & ... & N \\
JPSG031.997+00.067 & 31.998 & 0.068 & I & Y \\
JPSG032.012+00.057 & 32.009 & 0.058 & I & N \\
JPSG032.019+00.065 & 32.019 & 0.067 & II & Y \\
JPSG032.027+00.059 & 32.026 & 0.055 & ... & Y \\
JPSG032.037+00.056 & 32.036 & 0.056 & ... & Y \\
JPSG032.044+00.059 & 32.045 & 0.061 & ... & Y \\
JPSG032.062+00.071 & 32.060 & 0.073 & ... & Y \\
JPSG032.087+00.076 & 32.085 & 0.077 & ... & Y \\
JPSG032.097+00.076 & 32.097 & 0.075 & ... & Y \\
JPSG032.116+00.090 & 32.120 & 0.093 & ... & Y \\
JPSG032.141+00.172 & 32.142 & 0.172 & II & N \\
JPSG032.150+00.133 & 32.151 & 0.136 & II & Y \\
JPSG032.152+00.122 & 32.151 & 0.120 & ... & Y \\
JPSG032.160+00.113 & 32.161 & 0.114 & II & Y \\
JPSG032.164+00.171 & 32.163 & 0.172 & ... & N \\
JPSG032.170+00.135 & 32.170 & 0.135 & ... & Y \\
JPSG032.179+00.137 & 32.179 & 0.138 & ... & Y \\
\hline
\end{tabular}
\end{table*}


==> Catalogue/jps_gaspara.tex <==
\begin{table}
\begin{tabular}{ccccc}
\hline
JPS\_name & $l_{peak}$ & $b_{peak}$ & $T_{ex}$ & $N_{H2}$ \\
 & & & K & $cm^{-2}$ \\
\hline
JPSG031.925+00.083 & 31.925 & 0.083 & 13.30 & 1.78e+22 \\
JPSG031.929+00.056 & 31.929 & 0.056 & 14.12 & 1.39e+22 \\
JPSG031.933+00.090 & 31.933 & 0.090 & 12.51 & 1.72e+22 \\
JPSG031.945+00.076 & 31.945 & 0.076 & 13.50 & 2.04e+22 \\
JPSG031.951+00.071 & 31.951 & 0.071 & 14.43 & 2.37e+22 \\
JPSG031.961+00.066 & 31.961 & 0.066 & 15.27 & 2.45e+22 \\
JPSG031.965+00.062 & 31.965 & 0.062 & 15.27 & 2.45e+22 \\
JPSG031.970+00.060 & 31.970 & 0.060 & 15.61 & 2.69e+22 \\
JPSG031.984+00.065 & 31.984 & 0.065 & 16.24 & 3.33e+22 \\
JPSG031.991+00.067 & 31.991 & 0.067 & 17.35 & 3.67e+22 \\
JPSG031.997+00.067 & 31.997 & 0.067 & 17.17 & 3.93e+22 \\
JPSG032.012+00.057 & 32.012 & 0.057 & 17.17 & 4.54e+22 \\
JPSG032.019+00.065 & 32.019 & 0.065 & 20.26 & 6.25e+22 \\
JPSG032.027+00.059 & 32.027 & 0.059 & 21.12 & 6.63e+22 \\
JPSG032.037+00.056 & 32.037 & 0.056 & 18.58 & 5.35e+22 \\
JPSG032.044+00.059 & 32.044 & 0.059 & 19.88 & 5.20e+22 \\
JPSG032.062+00.071 & 32.062 & 0.071 & 20.96 & 3.19e+22 \\
JPSG032.087+00.076 & 32.087 & 0.076 & 18.77 & 2.44e+22 \\
JPSG032.097+00.076 & 32.097 & 0.076 & 16.03 & 2.16e+22 \\
JPSG032.116+00.090 & 32.116 & 0.090 & 18.07 & 2.84e+22 \\
JPSG032.141+00.172 & 32.141 & 0.172 & 12.97 & 1.33e+22 \\
JPSG032.150+00.133 & 32.150 & 0.133 & 20.87 & 3.12e+22 \\
JPSG032.152+00.122 & 32.152 & 0.122 & 20.54 & 2.61e+22 \\
JPSG032.160+00.113 & 32.160 & 0.113 & 17.95 & 1.62e+22 \\
JPSG032.164+00.171 & 32.164 & 0.171 & 11.72 & 1.44e+22 \\
JPSG032.170+00.135 & 32.170 & 0.135 & 16.39 & 1.92e+22 \\
JPSG032.179+00.137 & 32.179 & 0.137 & 16.39 & 1.92e+22 \\
\end{tabular}
\end{table}


==> Catalogue/jps_sedpara.tex <==
\begin{table*}
\caption{SED result}
\begin{tabular}{ccccccccccccc}
\hline \\
JPS\_name & l\_peak & b\_peak & maj & min & PA & r\_eff & T\_dust & N\_H2 & n\_H2 & S\_850 & SNR\_850 & Mass\_850 \\
 & & & \arcsec & \arcsec & \degr & pc & K & & & Jy & & $M_{\sun}$ \\
\hline \\
JPSG031.925+00.083 & 31.925 & 0.083 & 17 & 7 & 185 & 0.86 & 13.17 & 1.78e+22 & 4.77e+03 & 0.9 & 8.1 & 8.71e+02 \\
JPSG031.929+00.056 & 31.929 & 0.056 & 12 & 8 & 151 & 0.69 & 15.33 & 9.11e+21 & 3.67e+03 & 0.46 & 5.55 & 3.43e+02 \\
JPSG031.933+00.090 & 31.933 & 0.090 & 17 & 8 & 244 & 0.89 & 12.72 & 2.51e+22 & 4.61e+03 & 0.92 & 8.49 & 9.48e+02 \\
JPSG031.945+00.076 & 31.945 & 0.076 & 17 & 12 & 211 & 1.10 & 11.97 & 4.29e+22 & 5.89e+03 & 1.96 & 17.39 & 2.26e+03 \\
JPSG031.951+00.071 & 31.951 & 0.071 & 10 & 5 & 148 & 0.48 & 12.19 & 3.80e+22 & 1.53e+04 & 0.44 & 7.81 & 4.90e+02 \\
JPSG031.961+00.066 & 31.961 & 0.066 & 19 & 11 & 97 & 1.06 & 12.73 & 3.50e+22 & 4.67e+03 & 1.58 & 9.84 & 1.63e+03 \\
JPSG031.965+00.062 & 31.965 & 0.062 & 9 & 6 & 116 & 0.55 & 12.73 & 3.45e+22 & 1.42e+04 & 0.66 & 10.68 & 6.79e+02 \\
JPSG031.970+00.060 & 31.970 & 0.060 & 14 & 10 & 255 & 0.89 & 12.68 & 3.22e+22 & 5.95e+03 & 1.18 & 9.96 & 1.22e+03 \\
JPSG031.984+00.065 & 31.984 & 0.065 & 14 & 12 & 231 & 1.03 & 13.06 & 3.85e+22 & 6.13e+03 & 1.97 & 16.05 & 1.93e+03 \\
JPSG031.991+00.067 & 31.991 & 0.067 & 12 & 6 & 260 & 0.65 & 13.12 & 4.61e+22 & 1.19e+04 & 0.98 & 13.16 & 9.55e+02 \\
JPSG031.997+00.067 & 31.997 & 0.067 & 10 & 10 & 110 & 0.79 & 13.01 & 4.99e+22 & 1.17e+04 & 1.68 & 16.27 & 1.66e+03 \\
JPSG032.012+00.057 & 32.012 & 0.057 & 17 & 13 & 205 & 1.20 & 13.08 & 8.99e+22 & 1.11e+04 & 5.7 & 32.3 & 5.58e+03 \\
JPSG032.019+00.065 & 32.019 & 0.065 & 22 & 16 & 144 & 1.51 & 14.61 & 1.01e+23 & 7.15e+03 & 8.81 & 46.03 & 7.12e+03 \\
JPSG032.027+00.059 & 32.027 & 0.059 & 20 & 11 & 95 & 1.13 & 15.50 & 9.54e+22 & 1.07e+04 & 6.14 & 33.86 & 4.50e+03 \\
JPSG032.037+00.056 & 32.037 & 0.056 & 17 & 10 & 262 & 1.13 & 20.21 & 7.57e+22 & 9.39e+03 & 8.13 & 67.59 & 3.94e+03 \\
JPSG032.044+00.059 & 32.044 & 0.059 & 16 & 13 & 109 & 1.44 & 24.19 & 7.57e+22 & 6.06e+03 & 13.99 & 174.24 & 5.24e+03 \\
JPSG032.062+00.071 & 32.062 & 0.071 & 10 & 6 & 132 & 0.58 & 20.19 & 9.51e+21 & 4.06e+03 & 0.48 & 7.08 & 2.33e+02 \\
JPSG032.087+00.076 & 32.087 & 0.076 & 21 & 7 & 237 & 0.82 & 21.32 & 7.37e+21 & 1.53e+03 & 0.55 & 5.25 & 2.47e+02 \\
JPSG032.097+00.076 & 32.097 & 0.076 & 11 & 7 & 154 & 0.65 & 21.36 & 7.18e+21 & 2.45e+03 & 0.44 & 5.13 & 1.97e+02 \\
JPSG032.116+00.090 & 32.116 & 0.090 & 25 & 18 & 150 & 1.89 & 26.45 & 2.66e+22 & 1.46e+03 & 8.54 & 60.8 & 2.83e+03 \\
JPSG032.141+00.172 & 32.141 & 0.172 & 14 & 8 & 240 & 0.72 & 16.84 & 8.95e+21 & 2.90e+03 & 0.49 & 5.83 & 3.14e+02 \\
JPSG032.150+00.133 & 32.150 & 0.133 & 22 & 17 & 262 & 1.78 & 24.94 & 3.71e+22 & 2.89e+03 & 13.24 & 112.86 & 4.76e+03 \\
JPSG032.152+00.122 & 32.152 & 0.122 & 16 & 12 & 125 & 1.03 & 19.97 & 2.34e+22 & 4.10e+03 & 2.62 & 20.6 & 1.29e+03 \\
JPSG032.160+00.113 & 32.160 & 0.113 & 17 & 11 & 209 & 0.93 & 20.08 & 1.11e+22 & 2.47e+03 & 1.16 & 10.01 & 5.68e+02 \\
JPSG032.164+00.171 & 32.164 & 0.171 & 9 & 6 & 216 & 0.55 & 15.86 & 1.26e+22 & 4.72e+03 & 0.32 & 6.41 & 2.26e+02 \\
JPSG032.170+00.135 & 32.170 & 0.135 & 9 & 6 & 163 & 0.58 & 18.59 & 1.01e+22 & 4.98e+03 & 0.52 & 8.12 & 2.86e+02 \\
JPSG032.179+00.137 & 32.179 & 0.137 & 11 & 5 & 147 & 0.58 & 17.18 & 1.07e+22 & 3.79e+03 & 0.35 & 5.72 & 2.17e+02 \\
\hline 
\end{tabular}
\end{table*}

